Label-Imbalanced and Group-Sensitive Classification under Overparameterization

The goal in label-imbalanced and group-sensitive classification is to optimize relevant metrics such as balanced error and equal opportunity. Classical methods, such as weighted cross-entropy, fail when training deep nets to the terminal phase of training (TPT), that is training beyond zero training error. This observation has motivated recent flurry of activity in developing heuristic alternatives following the intuitive mechanism of promoting larger margin for minorities. In contrast to previous heuristics, we follow a principled analysis explaining how different loss adjustments affect margins. First, we prove that for all linear classifiers trained in TPT, it is necessary to introduce multiplicative, rather than additive, logit adjustments so that the interclass margins change appropriately. To show this, we discover a connection of the multiplicative CE modification to the cost-sensitive support-vector machines. Perhaps counterintuitively, we also find that, at the start of training, the same multiplicative weights can actually harm the minority classes. Thus, while additive adjustments are ineffective in the TPT, we show that they can speed up convergence by countering the initial negative effect of the multiplicative weights. Motivated by these findings, we formulate the vector-scaling (VS) loss, that captures existing techniques as special cases. Moreover, we introduce a natural extension of the VS-loss to group-sensitive classification, thus treating the two common types of imbalances (label/group) in a unifying way. Importantly, our experiments on state-of-the-art datasets are fully consistent with our theoretical insights and confirm the superior performance of our algorithms. Finally, for imbalanced Gaussian-mixtures data, we perform a generalization analysis, revealing tradeoffs between balanced / standard error and equal opportunity.

==> exp_copy.tex <==

%\op{I know we're sort on space but I think this table should be bigger, numbers are barely visible}
\begin{table}[]
   \caption{Top-1 accuracy results on balanced validation set ($\%$). Average of $5$ runs}
   \label{table:CIFAR}
    \begin{center}\resizebox{0.75\textwidth}{!}{
        \begin{tabular}{lllllllll} \hline
        \textbf{Dataset}         & \multicolumn{4}{c}{\textbf{CIFAR 10}} & \multicolumn{4}{c}{\textbf{CIFAR 100}} \\ \hline
        \textbf{Imbalance Type}  & \multicolumn{2}{c}{\textbf{LT}} & \multicolumn{2}{c}{\textbf{STEP}} & \multicolumn{2}{c}{\textbf{LT}} & \multicolumn{2}{c}{\textbf{STEP}} \\ \hline
        \textbf{Imbalance Ratio} & \textbf{100} & \textbf{10} & \textbf{100} & \textbf{10} & \textbf{100} & \textbf{10} & \textbf{100} & \textbf{10}     \\ \hline \hline
        CE                       						& 71.1  & 87.2  & 65.3  & 85.1  & 40.1  & 56.9  & 39.9  & 54.6 \\ 
        Re-Sampling              					& 71.2  & 86.5  & 65.0  & 84.5  & 34.7  & 54.2  & 38.4  & 52.1 \\ 
        wCE             							& 72.6  & 87.1  & 67.3  & 85.8  & 40.5  & 57.3  & 40.1  & 55.7 \\ \hline
        LDAM  \cite{TengyuMa}.                 			& 73.35 & 86.96 & 66.58 & 85.00 & 39.60 & 56.91 & 39.58 & 56.27 \\ 
        LDAM-DRW  \cite{TengyuMa}               		& 77.03 & 88.16 & 76.92 & 87.81 & 42.04 & 58.71 & 45.36 & \textbf{59.46} \\ 
        LA ($\tau=1$) \cite{Menon}                       		& 77.15 & 88.34 & 73.67 & 88.24 & 42.36 & 57.88 & \textbf{46.89} & 59.20 \\ 
        CDT ($\gamma=\gamma^{*}$)  \cite{CDT}         	& 79.22 & \textbf{88.76} & 73.26 & \textbf{89.00} & \textbf{42.95} & 57.85 & 42.36 & 59.40  \\ \hline \hline
        VS ($\tau=\tau^{*}, \gamma=\gamma^{*}$)             & \textbf{80.68} & 88.72 & \textbf{79.10} & 88.67 & 42.79 & \textbf{57.97} & 46.44 & 59.43
%        VS-DRW ($\tau=\tau^{*}, \gamma=\gamma^{*}$)   &       &        &       &       &       &       &      &       
\\ \hline
        \end{tabular}}
    \end{center}
\end{table}



\vspace{-0.1in}
\subsection{Label-imbalanced data}
%\op{I put in comments what I think that can be deferred to the SM, let me know what you think}
\noindent\textbf{Datasets:} 
%In addition to the experiments with synthetic data presented above, w
We evaluate the VS-loss on CIFAR-10 and CIFAR-100 \cite{krizhevsky2009learning}; specifcally, on imbalanced instances generated by  \cite{TengyuMa}.
%, {each containing $50$k training and $10$k test images of size $32 \times 32$, equally distributed in $10$ and $100$ classes respectively.} 
We study two types of imbalance. (1) \textit{STEP} imbalance \cite{Buda_2018}, reduces the number of training instances of half of the classes to a fixed size. (2) Long-tailed (\textit{LT}) imbalance \cite{cui2019classbalanced} exponentially decreases the number of training images across different classes. In both cases we define the imbalance ratio as $\rho = N_{\max}/ N_{\min} \in \{10, 100\}$, where $N_{\max}=\max_y{N_y}, N_{\min}=\min_y{N_y}$ and $N_y$ are the sample sizes of each class $y$. For consistency with \cite{he2016deep, TengyuMa, Menon, CDT} we keet the test set balanced and in addition to evaluating our models on it, we treat it as our validation set and use it to tune our hyperparameters. \red{In the SM we discuss a more practical hyperparameter tuning strategy using a validation set held out of the training set and we demonstrate that this approach achieves similar performance on the test set.} {Same as in \cite{he2016deep, TengyuMa, Menon, CDT} we augment the data by padding the images to size $40 \times 40$, flipping them horizontally at random and then random cropping them to their original size. More results on other datasets are in the SM.}
\\
\noindent\textbf{Model and Baselines:} 
We compare the VS-loss against several different state-of-the-art baselines: 
\textbf{(1) CE-loss} (standard cross-entropy). \textbf{(2) Re-Sampling}, where every training instance is assigned a ${\pi_y}^{-1}$ probability to be included in the batch. \textbf{(3) wCE}, weighted CE with weights $\omega_y = {\pi_y}^{-1}$. \textbf{(4) LDAM-loss} \cite{TengyuMa}, a special case of LA-loss where $\iota_y = \frac{1}{2} ({N_{\min}}/{N_y})^{1/4}$ is \emph{subtracted} from the logits.  \textbf{(5) LDAM-DRW} \cite{TengyuMa}, combining LDAM with deferred re-weighting (i.e. $\omega_y \neq 1$ only as we enter TPT). \textbf{(6) LA-loss} \cite{Menon}, with the Fisher-consistent parametric choice $\iota_y = \tau \log(\pi_y)$ added to the logits. \textbf{(7) CDT-loss} \cite{CDT}, where the logits are multiplied by $\Delta_y = ({N_{y}}/{N_{max}})^{\gamma}$. \textbf{(8) VS-loss}, with combined hyperparameters $\iota_y = \tau \log(\pi_y)$ and $\Delta_y = ({N_{y}}/{N_{\max}})^{\gamma}$, parameterized by $\tau, \gamma>0$ respectively.  We note that the three papers that first introduced (5), (6) and (7) above, all trained CIFAR for a different number of epochs and with dissimilar regularization and learning rate schedules. Here, for consistency, we follow the training setting by \cite{TengyuMa} (see below). Thus, for LDAM we show the results reported by \cite{TengyuMa}, but for the LA/CDT, we reproduce the results of \cite{Menon,CDT} in the above setting.
\\
\noindent\textbf{Technical details:} \red{We follow \cite{TengyuMa}.} We train a ResNet-32 model \cite{he2016deep}, using batch size $128$ and SGD with momentum $0.9$ and weight decay $2\times10^{-4}$. For the first $5$ epochs we use a linear warm up schedule until baseline learning rate of $0.1$. We train for a total of 200 epochs, while decaying our learning rate by $0.1$ at epochs $160$ and $180.$ We develop our code using PyTorch \cite{paszke2017automatic} building on codes provided by \cite{TengyuMa,CDT}. Training is performed on 2 NVIDIA RTX-3080 GPUs. \red{We remark that LDAM failed to converge in this setting, thus we used learning rate decay 0.01. For that same loss we also normalized the features norms after the last layer before the classifiers and the weights of the classifiers as done by \cite{TengyuMa}. We avoid that for the rest of the losses to isolate the impact of loss-modification which is our focus.}
% \op{One exception to that is LDAM which fails to converge in this setting and for which we use learning rate decay 0.01. For that same loss we must also normalize the features norms after the last layer before the classifiers and the weights of the classifiers.}
\\
\noindent\textbf{Results:} Table \ref{table:CIFAR} shows Top-1 accuracy results on the balanced validation set (averages over 5 runs) on CIFAR 10/100, for STEP/LT imbalances with imbalance-ratios 10 and 100. We tune $\gamma$ for the CDT-loss and both $\tau$ and $\gamma$ for the VS-loss on the validation set. \red{The best value found is denoted $\tau^*, \gamma^*$ repsectively (see SM).} We also evaluated the performance of VS-loss with DRW.  We see that the VS loss frequently outperforms other methods. In theory, as VS includes LA and CDT as special cases, it should always perform at least as good as them given that the optimal hyperparameters were chosen. However, we observe that in some cases VS performs slightly worse than these losses, that is because in practice the distribution of the validation set on which the hyperparameters were chosen differs from that of the test set. \op{Here the validation and the test set are the same, so the real reason here is that I don't use seeds, thus there is some randomness and over a small amount of runs LA and CDT can perform better than VS} Additional results, including histograms of the per class error rates and plots of the dynamics of training are included in the SM.


==> exp_figures.tex <==








==> groups.tex <==

%\vspace{-0.05in}
\subsection{Analysis of GS-SVM}\label{sec:sharp_GS}
%\vspace{-0.05in}
Now, we focus on the group-sensitive case to characterize the DEO of GS-SVM. 



%\vp
%\noindent\textbf{Data model:}~We consider a binary GMM with $K$. Group membership is decided conditionally on the label such that $\forall j\in[K],$ $\Pro\{g=j|y=+1\}=p_{+,j}$ and $\Pro\{g=j|y=-1\}=p_{-,j},$ with $\sum_{j\in[K]}p_{+,j}=\sum_{j\in[K]}p_{-,j}=1$. Within each class, each group is associated with a mean vector $\mub_{\pm1,j}=\pm\mub_{g}\in\R^d$ for positive/negative label respectively. Specifically, we let $\x\,|\,(y,g) \sim \Nn(y\mub_{g},\mathbf{I}_d)$.
%Denote $\M=\begin{bmatrix} \mub_{1} & \mub_{2}\end{bmatrix}$  and assume the  eigenvalue decomposition 
%$
%\M^T\M = \Vb\Sb^2\Vb^T, \Sb\succ \mathbf{0}_{r\times r},\Vb\in\R^{2\times r}, r\in\{1,2\}
%$.  For concreteness, we focus on two groups ($K=2$) with $p_{+,j}=p_{-,j}=p_j,\,j=1,2$ and group imbalance $p:=p_{1}< p_2=1-p$.

\textbf{Sharp asymptotics:}~First, we need the following definitions. Let $G,Y$ as defined in Sec. \ref{sec:CS-SVM_sharp}. Fix $\delta>0$. Define additional random variables $GS, \Delta_S\in\R,$ and $E_{S}\in\R^{2\times 1}$ as follows: 
 Fix $\delta>0$. Define random variables $G, Y, S, \Delta_S\in\R,$ and $E_{S}\in\R^{2\times 1}$ as follows: 
\begin{equation*}
\begin{cases}
%~G\sim \Nn(0,1), \quad \text{$Y$ symmetric Bernoulli with $\Pro\{Y=+1\}=\pi$}\\
~\text{$S$ takes values $1$ or $2$ with probabilities $p$ and $1-p$, respectively}\\
~E_{S}=\eb_1\ind{S=1}+\eb_2\ind{S=2}\quad\text{and}\quad\Delta_S=\delta\cdot\ind{S=1} +1\cdot\ind{S=2},
\end{cases}
\end{equation*} 
and function $\wtd\eta_\delta:\R_{\geq0}\times\Bc_2^{r}\times\R\rightarrow\R$ as 
$
		%&\eta_\delta(\qt,\rhobt,\bt):=
		\wtd\eta_\delta(q_\delta,\rhob_\delta,b_\delta):=\E\big(G+E_{S}^T\Vb\Sb\rhobt + \frac{\bt Y-\Delta_S}{\qt}\big)_{-}^2 \nn- (1-\|\rhobt\|_2^2)\gamma.
$


%Hence, we may use the VS-loss in \eqref{eq:loss_ours_bin_group} with $\Delta_{y,g}=\Delta_{g}$ for $g=1,2$.  In particular, since we are interested on separable data,  we will focus on the GS-SVM in \eqref{eq:GS-SVM} (where similar to Proposition \ref{propo:gd} for label imbalances, we map $\delta=\Delta_2/\Delta_1$).


\begin{theorem}[Equal Opportunity of GS-SVM]\label{thm:main_group_fairness}
Let the data model and learning regime as described above. 
Consider the GS-SVM classifier with $h(\x)=\x$, intercept $b$ and fixed margin-ratio $\delta>0$ (corresponding to group VS-loss with $\Delta_{y,g}=\Delta_{g}, g=1,2$ such that $\delta=\Delta_2/\Delta_1$).
%Consider the GMM with feature distribution and priors as specified in the `Data model' above. 
	Let $(\wtd q_\delta,\wtd \rhob_\delta, \wtd b_\delta)$ be the unique triplet satisfying same equations as in Theorem \ref{thm:main_imbalance}, but with $\eta_\delta$ replaced with the function $\wtd \eta_\delta$ above. 
%	equation
%	\begin{align}\label{eq:eta_eq}
%		\min_{\substack{\|\rhobt\|_2\leq 1,\, \bt\in\R}}\eta_\delta(\qt,\rhobt,\bt) = 0\,,
%	\end{align}
%	and $\rhob,b$ be the unique minimizers of $\eta_\delta(q,\rhobt,\bt)$. 
Then, in the limit of $n,d\rightarrow\infty, d/n=\gamma>\wtd\gamma_{\star}$ it holds 
$
\Rc_{\pm,i} \rP Q\big({\eb_i^T\Vb\Sb\wtd \rhob_\delta\pm \wtd b_\delta/{\wtd q_\delta}}\big), i=1,2.$ In particular, the difference of equal opportunity (DEO) satisfies 
$
\Rc_{\rm deo} \rP Q\big({\eb_1^T\Vb\Sb\wtd \rhob_\delta+ \wtd b_\delta/{\wtd q_\delta}}\big) - Q\big({\eb_2^T\Vb\Sb\wtd \rhob_\delta+ \wtd b_\delta/{\wtd q_\delta}}\big).$
\end{theorem}

The proof (given in the SM) differs to that of Theorem \ref{thm:main_imbalance} since now each class itself is a mixture of Gaussians. 


\noindent\textbf{Tradeoffs:}~Our theorem allows us to study tradeoffs between DEO and accuracy  in Fig. \ref{fig:fairness_deo_misclas_tradeoff}(b). Specifically, we investigate the effect of $\delta$ and the improvement of  GS-SVM over standard SVM (corresponding to $\delta=1$). The largest DEO and smallest misclassification error are achieved by the SVM ($\delta=1$). But, with increasing $\delta$, misclassification error is traded-off for reduction in absolute value of DEO. Interestingly, for some $\delta_0=\delta_0(\gamma)$ (with value increasing as function of $\gamma$) GS-SVM guarantees Equal Opportunity (EO) $\Rc_{\rm deo}=0$ (without explicitly imposing such constraints as in \cite{olfat2018spectral,donini2018empirical}). 

%In view of the formulas, the requirement for EO translates to  finding a parameter $\delta_0$ such that $Q\big({\eb_1^T\Vb\Sb\wtd \rhob_{\delta_0} +  \wtd b_{\delta_0}/{\wtd q_{\delta_0}}}\big)=Q\big({\eb_2^T\Vb\Sb\wtd \rhob_{\delta_0} +  \wtd b_{\delta_0}/{\wtd q_{\delta_0}}}\big)$. While, we cannot find an explicit formula (as we did for $\delta_\star$ in \eqref{eq:delta_star}), we can search for $\delta_0$ numerically. Interestingly, Figure \ref{fig:fairness_deo_misclas_tradeoff} shows that such values exist in our setting even though the GS-SVM does not directly impose EO constraints as several related works, e.g. \cite{olfat2018spectral,donini2018empirical}.
%The proof of Theorem \ref{thm:main_group_fairness}, which is similar to that of Theorem \ref{thm:main_imbalance}, is presented in Appendix \ref{sec:gs-svm_proof}.




%\begin{theorem}\label{thm:main_group_fairness}
%Consider the GMM with two groups $K=2$ and with feature distribution and priors as specified in the `Data model' above. Fix $\delta>0$. Define random variables $G, Y, S, \Delta_S\in\R, Z_S$ and $E_{S}\in\R^{2\times 1}$ as follows: 
%$G\sim \Nn(0,1)$; $Y$ is a symmetric Bernoulli with $\Pro\{Y=+1\}=\pi$;  $S$ takes values $1$ or $2$ with probabilities $p$ and $1-p$, respectively; 
% $E_{S}=\eb_1\ind{S=1}+\eb_2\ind{S=2}$; $\Delta_S=\delta\cdot\ind{S=1} +1\cdot\ind{S=2}$; and, $Z_S=\sigma_1^{-2}\cdot\ind{S=1} +\sigma_2^{-2}\cdot\ind{S=2}$ . With these define function $\wt\eta_\delta:\R_{\geq0}\times\Sc^{r}\times\R\rightarrow\R$:
%\begin{align}
%%&\eta_\delta(\qt,\rhobt,\bt):=
%\E\big(G+Z_SE_{S}^T\Vb\Sb\rhobt + Z_S\frac{\bt Y-\Delta_S}{\qt}\big)_{-}^2 \nn- (1-\|\rhobt\|_2^2)\gamma.
%\end{align}
%Let $q$ be the unique solution of the equation
%\begin{align}\label{eq:eta_eq}
%\min_{\substack{\|\rhobt\|_2\leq 1,\, \bt\in\R}}\eta_\delta(\qt,\rhobt,\bt) = 0\,,
%\end{align}
%and $\rhob,b$ be the unique minimizers of $\eta_\delta(q,\rhobt,\bt)$. Then, in the limit of $n,d\rightarrow\infty$ with $d/n=\gamma>\gamma_{\star,g}$ it holds that
%\begin{align*}
%\Rc_{+,1} &\rP Q\Big(\frac{\eb_1^T\Vb\Sb\rhob+b/q}{\sigma_1}\Big)\,,~~
%\Rc_{+,2} \rP Q\Big(\frac{\eb_2^T\Vb\Sb\rhob+b/q}{\sigma_2}\Big)\,,\\
%\Rc_{-,1} &\rP Q\Big(\frac{-\eb_1^T\Vb\Sb\rhob-b/q}{\sigma_1}\Big)\,,~~
%\Rc_{-,2} \rP Q\Big(\frac{-\eb_2^T\Vb\Sb\rhob-b/q}{\sigma_2}\Big).
%\end{align*}
%
%\ct{formulas for orthogonal $\mub_1,\mub_2$.}
%\ct{Specialize to $\mub_1=[\mub;\mub], \mub_2=[\mub;-\mub]$}
%
%% $\{\min\eta(q,\rho_+,\rho_{-},b)~:~\rho_+\in[-1,1],\rho_-\in[-1,1],b\in\R\}$
%%\begin{align*}
%%&G\sim\Nn(0,1) 
%%\quad Y=\begin{cases} +1 &, \text{w.p. } \pi \\ -1 &, \text{w.p. } 1-\pi\end{cases} 
%%\\
%%&\Delta_Y=\begin{cases} +1 &, \text{w.p. } \pi \\ -1 &, \text{w.p. } 1-\pi\end{cases}
%%\end{align*}
%%$G\sim\Nn(0,1)$, $Y$ be a symmetric Bernoulli random variable with $\Pro{Y=+1}=\pi$ $Y=\begin{cases} +1 &, \text{w.p. } \pi \\ -1 &\text{w.p. } 1-\pi\end{cases}$
%\end{theorem}
%

==> loss.tex <==
\section{What is going on with the loss?!}

Let the label set $\Yc=\{1,2,\ldots,K\}$ for a K-class classification setting and consider the cross-entropy VS-loss:
\begin{align}\label{eq:loss_app_multi_A}
\Lc(\W)&:= -\sum_{i\in[n]}\om_{y_i}\log\left(\frac{e^{\Delta_{y_i}\w_{y_i}^T\x+\iota_{y_i}}}{\sum_{c\in[K]}e^{\Delta_{y_i}\w_c^T\x+\iota_c}}\right)
\\
&=\sum_{i\in[n]}\om_{y_i}\log\Big(1+\sum_{\substack{y'\in[K]\\y'\neq y_i}}e^{\iota_{y'}-\iota_{y_i}}e^{- \Del_{y_i} (\w_{y_i}^T\x_i-\w_{y'}^T\x_i)}\Big),\nn
\end{align}
where $\W=[\w_1,\ldots,\w_K]\in\R^{K\times d}$ and $\w_y$ is the classifier corresponding to class $y\in[K]$. The VS-loss converges to the following CS $K$-class SVM:
\begin{align}\label{eq:CS-SVM_app_multi_A}
\boxed{\hat\W = \arg\min_{\W} \|\W\|_F\quad\text{subject to }\Delta_{y_i}\x_i^T(\w_{y_i}-\w_{y'})\geq 1, ~\forall y'\neq y_i\in[K]~\text{ and }~\forall i\in[n].}
\end{align}

Now consider the other loss
\begin{align}\label{eq:loss_app_multi_A_2}
\Lc(\W)&:= -\sum_{i\in[n]}\om_{y_i}\log\left(\frac{e^{\Delta_{y_i}\w_{y_i}^T\x+\iota_{y_i}}}{\sum_{c\in[K]}e^{\Delta_c\w_c^T\x+\iota_c}}\right)
\\
&=\sum_{i\in[n]}\om_{y_i}\log\Big(1+\sum_{\substack{y'\in[K]\\y'\neq y_i}}e^{\iota_{y'}-\iota_{y_i}}e^{- (\Del_{y_i}\w_{y_i}-\Delta_{y'}\w_{y'})^T\x_i)}\Big)
\end{align}
This loss converges to the following
\begin{align}\label{eq:CS-SVM_app_multi_A_2}
\boxed{\hat\W = \arg\min_{\W} \|\W\|_F\quad\text{subject to }(\Delta_{y_i}\w_{y_i}-\Delta_{y'}\w_{y'})^T\x_i\geq 1, ~\forall y'\neq y_i\in[K]~\text{ and }~\forall i\in[n].}
\end{align}

\subsection{Binary case}
Consider the binary case: $y_i=\pm1$.

\vp
\noindent$\bullet$~~\eqref{eq:CS-SVM_app_multi_A} becomes
\begin{align}
\min \|\w_+\|_2^2 + \|\w_-\|_2^2\quad\text{subject to } \begin{cases}
\Delta_+(\w_+-\w_-)^T\x_i\geq 1 & y_i=+1 \\
\Delta_-(\w_--\w_+)^T\x_i\geq 1 & y_i=-1
\end{cases}
\end{align}
Change variables to $\vb=\w_+-\w_-$ and $\ub=\w_++\w_-$. Note that 
$$
\|\w_+\|_2^2 + \|\w_-\|_2^2 = \frac{1}{4}\|\vb+\ub\|_2^2 + \frac{1}{4}\|\vb-\ub\|_2^2 = \frac{1}{2}\|\vb\|_2^2+\frac{1}{2}\|\ub\|_2^2.
$$
Thus, the above reduces to 
\begin{align}
\min \|\vb\|_2^2 + \|\ub\|_2^2\quad\text{subject to } \begin{cases}
\Delta_+\vb^T\x_i\geq 1 & y_i=+1 \\
-\Delta_-\vb^T\x_i\geq 1 & y_i=-1
\end{cases} \qquad = \qquad 
\min \|\vb\|_2^2 \quad\text{subject to } 
y_i\Delta_{y_i}\vb^T\x_i\geq 1 
\end{align}
Recognize that the latter is exactly the binary CS-SVM.
To conclude, letting $\vb_{\rm CS-SVM}$ be the corresponding CS-SVM solution, we have shown that 
$$
\w_+=-\w_-={\vb_{\rm CS-SVM}}/{2},
$$
So, decision rule for a new sample $\x$ is $\hat y=\arg\max_{y=\pm} \w_y^T\x=\rm{sign}((\w_+-\w_-)^T\x)=\rm{sign}(\vb_{\rm CS-SVM}^T\x)$.

\vp
\noindent$\bullet$~~\eqref{eq:CS-SVM_app_multi_A_2} becomes
\begin{align}
\min \|\w_+\|_2^2 + \|\w_-\|_2^2\quad\text{subject to } \begin{cases}
(\Delta_+\w_+-\Delta_-\w_-)^T\x_i\geq 1 & y_i=+1 \\
(\Delta_-\w_--\Delta_+\w_+)^T\x_i\geq 1 & y_i=-1
\end{cases}
\end{align}
Change variables to $\vb=\Delta_+\w_+-\Delta_-\w_-$ and $\ub=\Delta_+\w_++\Delta_-\w_-$.
Compute 
$$
\|\w_+\|_2^2 + \|\w_-\|_2^2 = \frac{1}{4\Delta_+^2}\|\vb+\ub\|_2^2 + \frac{1}{4\Delta_-^2}\|\vb-\ub\|_2^2 = \frac{\alpha}{2}\|\vb\|_2^2 +  \frac{\alpha}{2}\|\ub\|_2^2 + \beta\vb^T\ub
$$
with $\alpha=\frac{1}{\Delta_+^2}+\frac{1}{\Delta_-^2}$ and $\beta=\frac{1}{2\Delta_+^2}-\frac{1}{2\Delta_-^2}$.
Note then that the minimization over $\ub$ is unconstrained leading to the objective:
$$
\frac{\alpha}{2}\|\vb\|_2^2 - \frac{\beta^2}{2\alpha}\|\vb\|_2^2 = \frac{1}{2\alpha}(\alpha^2-\beta^2)\|\vb\|_2^2
$$
Thus, the optimization is equivalent to 
\begin{align}
\min~\|\vb\|_2^2\quad\text{subject to } y_i\x_i^T\vb\geq 1
\end{align}
which is of course nothing but standard SVM. To conclude, letting $\vb_{\rm SVM}$ be the corresponding CS-SVM solution, we have shown that 
$$
\w_+=\frac{1}{2\Delta_+}(\ub+\vb)= \frac{1}{2\Delta_+}(1-\beta/\alpha)\vb_{\rm SVM}\quad\text{and}\quad\w_-=\frac{1}{2\Delta_-}(\ub-\vb)= -\frac{1}{2\Delta_-}(1+\beta/\alpha)\vb_{\rm SVM}.
$$
So, decision rule for a new sample $\x$ is $\hat y=\arg\max_{y=\pm} \w_y^T\x=\rm{sign}((\w_+-\w_-)^T\x)=\rm{sign}(\vb_{\rm SVM}^T\x)$.

%\ct{But need to bring it back to the $\w_+$ and $\w_-$. Check this, we can write both in terms of SVM solution?}



==> story.tex <==
\section{Story}

\subsection{Contributions}
\subsubsection{Insights on state-of-the-art methods}

Tons of recent papers on how to mitigate imbalances. Mostly methods based on interesting, but heuristic/empirical, observations. Here, we give theoretical intuitions on some of the key findings. Later, we use the insights towards algorithmic contributions.

\vp
\noindent$\bullet$~\textbf{Multiplicative vs additive scalings (or LA vs CDT):}
Ye at al. introduce the CDT and report significant improvements over LA \ct{@Orestis,Ganesh: can we please check here how/if their reported numbers compare to those in the Google paper? Since Google paper never compares to them.}. Here, we offer a theoretical explanation on what multiplicative logit corrections can offer over additive ones. 
We prove that for binary linear classifiers multiplicative is advantageous over additive. We show this via a connection to cost-sensitive SVMs. In short, our key finding is that for overparameterized binary linear classifiers LA=CE=SVM and CDT=CS-SVM. Intuitively, CS-SVM is better than SVM. We prove this to be the case for a stylized Gaussian-mixtures dataset.

\vp
\noindent$\bullet$~\textbf{CE fails in group-case} Sagawa et al. argue and demonstrate empirically that CE loss fails in the presence of group-imbalances. We propose a natural extension of the CDT, called GDT, and we prove that GDT=GS-SVM where GS-SVM is the natural counterpart of CS-SVM for the group case that pushes decision boundary towards dominant groups. We analytically showcase the efficacy of GS-SVM (and thus GDT) in a stylized group-GMM.


\vp
\noindent$\bullet$~\textbf{Cost-sensitive methods can improve standard accuracy:} Cost-sensitive methods are typically designed to improve balanced accuracy. Empirically it has been reported (Khan et al. \cite{cosen} \ct{@Ganesh: can you please add the new citations})\gk{added} that they can also improve standard accuracy as a byproduct. Motivated by this, for the GMM we compute the fundamental tradeoff achieved by binary CDT loss between standard and balanced accuracy identifying scenarios where the empirical observations are confirmed. Perhaps surprisingly, we also prove for the same model that the tuning of CDT minimizing balanced error automatically balances the minority/majority errors. Talk about DEO here. That you can achieve zero.
 




\subsubsection{Algorithmic contributions}


\noindent$\bullet$~\textbf{VS loss (aka LA + CDT)}
\begin{itemize}
\item \ct{Hopefully Oresti's Credit Fraud experiment is a first example here}
\item \ct{Can we do a CIFAR 10 experiment where we simply combine best $\Delta$'s of CDT paper with best $\iota$'s of Menon/Google paper and hopefully show better balanced accuracy. If we show one such \textbf{benchmark} example we are golden.}
\end{itemize}

\vp
\noindent$\bullet$~\textbf{VS loss for group imbalances}
\begin{itemize}
\item \ct{Here any improvement over ERM is new, so we don't have to fight to show VS>LA. Just VS (with any combination of $\Delta$'s/$\iota$'s) is better than ERM. We need again one \textbf{DNN} example.}
\end{itemize}

\subsection{Discussion}

Our analysis offers  useful insights to existing methods. We hope that our work motivates further similar investigations as there admittedly remain many open questions towards navigating the zoo of recently proposed methods for learning under imbalances. Below we discuss some of the most fascinating to us and how they relate to our work.

\vp
\noindent$\bullet$~\textbf{Learned representations vs hand-crafted features:} To the best of our knowledge, our result is the first to theoretically justify the benefit of multiplicative weights. We do this in a linear setting, but most importantly assuming \emph{fixed} feature representations (perhaps through some kernel method). In particular this means that the distribution of the training samples is same as that of test samples. On the other hand,  \cite{ye2020identifying} (but also see \cite{kimkim_adjusting}) introduce CDT motivated by an empirical finding that the distributions of the \emph{learned feature representations} differ between training and test. Our implicit-bias theory does not extend to this setting and it would be fascinating extending to this direction (perhaps following  \cite{mixon2020neural}).

\vp
\noindent$\bullet$~\textbf{LA vs CDT redux:}  Why is still LA better than CE? Understand training dynamics. Empirically, we find that VS-loss is more unstable. Why?

\vp
\noindent$\bullet$~\textbf{Multiclass vs binary:} 

%%\vspace{-0.3in}
\section{Introduction}
%%\vspace{-0.1in}
%
%\vp
%\noindent $\bullet$~\textbf{A new \emph{vector-scaling} loss:} We propose the following \emph{vector-scaling} loss ({\color{red}\emph{VS-loss}}, in short):
%%%\vspace{-0.05in}
%\begin{align}\label{eq:loss_ours}
%\ell(y,f(\x)) &= \omega_y \,\log(1+\sum_{y'\neq y}{e^{\iota_{yy'}}\, e^{{\color{red}\Delta_{y}}(f_{y'}(\x)-f_y(\x))}})\,,
%%\\
%%&= -\omega_y \,\log\frac{e^{{\color{red}\Delta_y}f_y(\x)+\iota_y}}{\sum_{y'\in[k]}e^{{\color{red}\Delta_{y}}f_{y'}(\x)+\iota_{y'}}}\,,\nn
%%%\vspace{-0.01in}
%\end{align}
%as a modification of standard cross-entropy loss \footnote{For the specific choice $\iota_{yy'}=\iota_{y'}-\iota_y$ (e.g. \cite{Menon}), \eqref{eq:loss_ours} is equivalent to  $ \ell(y,f(\x)) = -\omega_y \,\log\frac{e^{{\color{red}\Delta_y}f_y(\x)+\iota_y}}{\sum_{y'\in[k]}e^{{\color{red}\Delta_{y}}f_{y'}(\x)+\iota_{y'}}}.$} appropriate for imbalanced $k$-class datasets. In addition to the weights $\omega_y$ and to the label-dependent offset parameters $\iota_{yy'}$ in \eqref{eq:loss_Menon}, the VS-loss in \eqref{eq:loss_ours} introduces \emph{multiplicative} scaling factors $\Delta_y>0$ to the margins (in red for emphasis). Both theoretically and empirically we demonstrate the beneficial role of these new parameters when training continues in the zero training-error regime.


%\vspace{-0.05in}
\vp
\noindent $\bullet$~\textbf{Connection to cost-sensitive SVM:} 
%We focus on binary classification. 
For  linear predictors and separable datasets, we argue that optimizing the loss in \eqref{eq:loss_Menon} with gradient descent leads to a classifier whose direction converges to the max-margin SVM solution \emph{irrespective} of the choice of the parameters $\omega_y$ and $\iota_y$. Instead, the VS loss leads to the solution of another old friend: the \emph{cost-sensitive SVM (CS-SVM)}. For binary classification (i.e. $y\in\{\pm1\}$), in particular, the resulting CS-SVM is parameterized by a \emph{margin-ratio parameter} $\delta=\Delta_{-1}/\Delta_{+1}$; see \eqref{eq:CS-SVM}. %For multiclass classification
% proposed in \cite{} as an alternative to (standard) SVM that favors ($\delta$ times) larger margin for the minority class. 

%\vspace{-0.05in}
\vp
\noindent $\bullet$~\textbf{CS-SVM through a modern lens:} For an insightful Gaussian mixtures model (GMM), we present formulae that sharply predict the classification and balanced errors of CS-SVM (and thus, of the VS-loss as well) in a \emph{high-dimensional} separable regime. Our formulae are explicit in terms of data geometry, class priors, parameterization ratio and tuning parameter $\delta$. 
%We also use this characterization to pose the problem of optimally tuning the margin-ratio parameter to minimize the balanced error as a deterministic nonlinear optimization. 
Additionally, we identify a key structural property of CS-SVM that together with our asymptotic theory lead to an explicit formula for the optimal margin ratio $\delta_\star$ that minimizes the balanced error. For example, we show that $\delta_\star$ not only depends on the class priors, but is also sensitive to the parameterization ratio.

%\vspace{-0.05in}
\vp
\noindent $\bullet$~\textbf{Group-sensitive SVM:} We propose natural modifications to \eqref{eq:loss_ours} and to CS-SVM for classification in the presence of sensitive groups. We then extend the GMM to capture the presence of imbalanced groups, and for binary labels we develop a sharp analysis of our algorithms under sufficient overparameterization. %\gk{We consider a scenario where the group-assignments of the training examples are known.}

%In this work, we make multiple key contributions to the topics of imbalanced and fair learning in the overparameterized regime.
%
%\noindent $\bullet$ \textbf{Unified approach to imbalanced \& fair classification:} 
%
%\noindent $\bullet$ \textbf{Insightful asymptotic analysis:} 
%
%\noindent $\bullet$ \textbf{Group-Sensitive SVM:} 

%\vspace{-0.05in}
\vp
\noindent $\bullet$ \textbf{Numerical experiments:} We present numerical experiments that corroborate our findings above. Also, using our sharp analysis we study key tradeoffs between balanced error / equal opportunity and misclassification error.



==> synthetic_Christos.tex <==
\subsection{VS-loss vs LA-loss for a synthetic GMM (Additional results on the experiment of Figure \ref{fig:mismatch_intro})}

In Figure \ref{fig:figure_intro_more} we have implemented the same experiment as in Figure \ref{fig:mismatch_intro} detailed in Section \ref{sec:example_imbalance}. Here, additionally to the balanced error in Figure \ref{fig:mismatch_intro}, we present results for the misclassification error and the two conditional errors. In all cases, we report both the results of Monte Carlo simulations, as well as, the theoretical formulas predicted by Theorem \ref{thm:main_imbalance}. As promised, the theorem sharply predicts the conditional error probabilities of both the minority and the majority class. Note the almost perfect match with the numerical averages despite the relatively small problem dimension ($d=300$). 

As noted in Section \ref{sec:example_imbalance}, we observe in the `Top Left' of the  figure that the VS-loss results in a better balanced error in the separable regime (where $\Rc_{\rm train}=0$) compared to the LA-loss. This naturally comes at a cost, as the role of the two losses is reversed in terms of the misclassification error (see `Top Right'). The two bottom figures explain these observations showing that VS-loss sacrifices the error of majority class for a significant drop in the error of the minority class. All types of errors decrease with increasing overparameterization ratio $\gamma$ due to the mispecified model; see also \cite{hastie2019surprises,deng2020model}.

For the numerical experiments in Figure \ref{fig:figure_intro_more} we minimized the VS-loss and the LA-loss in the separable regime using normalized gradient descent. Specifically, we use an in increasing learning rate that is appropriately normalized by the norm of the loss gradient for faster convergence. Please refer to Figure \ref{fig:normalized_gd_experiments} and Section \ref{sec:gd_num_app} for a discussion on the advantage of this over a constant learning rate.

\begin{figure}[t]
 \centering
         \includegraphics[width=0.6\textwidth,height=0.4\textwidth]{Figures/Appendix/details_synthetic_Christos.eps}
%\begin{subfigure}[b]{0.48\textwidth}
%         \centering
%         \includegraphics[width=0.7\textwidth,height=0.5\textwidth]{Figures/Appendix/details_synthetic_Christos_balanced.eps}
%%                  \caption{VS-loss vs CS-SVM}
%\end{subfigure}
%\begin{subfigure}[b]{0.48\textwidth}
%         \centering
%         \includegraphics[width=0.7\textwidth,height=0.5\textwidth]{Figures/Appendix/details_synthetic_Christos_standard.eps}
%%         \caption{LA-loss vs SVM}
%\end{subfigure}
%\\
%\begin{center}
%\begin{subfigure}[b]{0.48\textwidth}
%         \centering
%         \includegraphics[width=0.7\textwidth,height=0.5\textwidth]{Figures/Appendix/details_synthetic_Christos_maj.eps}
%%                  \caption{VS-loss vs CS-SVM}
%\end{subfigure}
%\begin{subfigure}[b]{0.48\textwidth}
%         \centering
%         \includegraphics[width=0.7\textwidth,height=0.5\textwidth]{Figures/Appendix/details_synthetic_Christos_minf.eps}
%%         \caption{LA-loss vs SVM}
%\end{subfigure}
%\end{center}
\caption{Performance of the VS-loss vs the Logt-adjusted loss for a GMM with missing features. The experimental setting is identical to that of Figure \ref{fig:mismatch_intro}. \emph{Top Left:} balanced error $\Rcbal$ and training error $\Rc_{\rm train}$ (in dashed lines). \emph{Top Right:} misclassification error $\Rc$. \emph{Bottom Left:} majority class error $\Rc_-$. \emph{Bottom Right:} minority class error $\Rc_+$. Solid lines correspond to theoretical formulas obtained thanks to Theorem \ref{thm:main_imbalance}.}
\label{fig:figure_intro_more}
\end{figure}


==> table_Orestis.tex <==
\begin{table}[]
   \caption{Top-1 accuracy results on the balanced validation set ($\%$)}
   \label{table:CIFAR}
    \begin{center}\resizebox{0.75\textwidth}{!}{
        \begin{tabular}{lllllllll} \hline
        \textbf{Dataset}         & \multicolumn{4}{c}{\textbf{CIFAR 10}} & \multicolumn{4}{c}{\textbf{CIFAR 100}} \\ \hline
        \textbf{Imbalance Type}  & \multicolumn{2}{c}{\textbf{LT}} & \multicolumn{2}{c}{\textbf{STEP}} & \multicolumn{2}{c}{\textbf{LT}} & \multicolumn{2}{c}{\textbf{STEP}} \\ \hline
        \textbf{Imbalance Ratio} & \textbf{100} & \textbf{10} & \textbf{100} & \textbf{10} & \textbf{100} & \textbf{10} & \textbf{100} & \textbf{10}     \\ \hline \hline
        CE                       						& 71.1  & 87.2  & 65.3  & 85.1  & 40.1  & 56.9  & 39.9  & 54.6 \\ 
        Re-Sampling              					& 71.2  & 86.5  & 65.0  & 84.5  & 34.7  & 54.2  & 38.4  & 52.1 \\ 
        wCE             							& 72.6  & 87.1  & 67.3  & 85.8  & 40.5  & 57.3  & 40.1  & 55.7 \\ \hline
        LDAM  \cite{TengyuMa}.                 			& 73.35 & 86.96 & 66.58 & 85.00 & 39.60 & 56.91 & 39.58 & 56.27 \\ 
        LDAM-DRW  \cite{TengyuMa}.               		& 77.03 & 88.16 & 76.92 & 87.81 & 42.04 & 58.71 & 45.36 & 59.46 \\ 
        LA ($\tau=1$) \cite{Menon}                       		& (80.97) & 88.47 & (77.88) & (88.92) & (40.53) & (57.74) & (43.24) & (57.02) \\ 
        CDT ($\gamma=\gamma^{*}$)  \cite{CDT}         	& 80.61 & 88.82 & 73.75 & 89.30 & 43.95 & 58.29 & 44.08 & 58.68  \\ \hline \hline
        VS ($\tau=\tau^{*}, \gamma=\gamma^{*}$)         & 81.10 & 88.84 & 79.83 & 89.88 & 43.95 & 58.65 & 46.72 & 58.72 \\ 
        \end{tabular}}
    \end{center}
\end{table}

==> thm_gssvm_app.tex <==
\section{Generalization Analysis for Group-VS-loss / GS-SVM}\label{sec:thm_gssvm_app}
In Theorem \ref{thm:main_imbalance}, we stated a sharp asymptotic theoretical result for VS-loss/CS-SVM under the Gaussian mixture data model. Here, we will state the counterpart result for GS-SVM with an appropriate Gaussian mixture data model with group imbalances. 
\\
\noindent\textbf{Data model:}~We study a binary Gaussian-mixture generative model (GMM) for the data distribution $\Dc$. For the label $y\in\{\pm1\}$ let $\pi:=\Pro\{y=+1\}.$ Group membership is decided conditionally on the label such that $\forall j\in[K]:$ $\Pro\{g=j|y=\pm1\}=p_{\pm,j}$, with $\sum_{j\in[K]}p_{+,j}=\sum_{j\in[K]}p_{-,j}=1$. Finally, the feature conditional given label $y$ and group $g$ is a multivariate Gaussian of mean $\mub_{y,g}\in\R^d$ and covariance $\Sigmab$, that is, 
$\x\big|(y,g)\,\widesim{} \Nn(\mub_{y,g},\Sigmab).
$
%For \emph{label-imbalances}, we assume all examples belong to the same group ($K=1$),  and an imbalanced setting in which $\pi\ll1-\pi$. 
We focus on two groups $K=2$ with $p_{+,1}=p_{-,1}=p<1-p=p_{+,2}=p_{-,2},\,j=1,2$ and $\x\,|\,(y,g) \sim \Nn(y\mub_{g},\mathbf{I}_d)$. As before, let $\M$ denote the matrix of means (that is $\M=\begin{bmatrix} \mub_{+} & \mub_{-}\end{bmatrix}$ and $\M=\begin{bmatrix} \mub_{1} & \mub_{2}\end{bmatrix}$, respectively) and consider the eigen-decomposition of its Gramian:
$
\M^T\M = \Vb\Sb^2\Vb^T,~~ \Sb\succ \mathbf{0}_{r\times r},\Vb\in\R^{2\times r}, r\in\{1,2\},
$
with $\Sb$ an $r\times r$ diagonal positive-definite matrix and $\Vb$ an orthonormal matrix obeying  $\Vb^T\Vb=\mathbf{I}_r$. We study linear classifiers with $h(\x)=\x$. 
\\
\noindent\textbf{Learning regime:}~%We study the proportional high-dimensional regime in which both sample size $n$ and feature dimension $d$ grow to infinity at a fixed rate $\gamma=d/n$.
Again, as in Theorem \ref{thm:main_imbalance}, we focus on a regime where training data are linearly separable. It turns out once again that linear separability undergoes a sharp phase-transition as $d,n\rightarrow\infty$ at a proportional rate $\gamma=\frac{d}{n}$. There exists threshold $\wtd\gamma_{\star}:=\wtd\gamma_{\star}(\Vb,\Sb,\pi,p)\leq 1/2$, such
that data are linearly separable with probability approaching one provided that $\gamma>\wtd\gamma_{\star}$ \cite{candes2020phase,montanari2019generalization,deng2019model,kammoun2020precise,gkct_icassp}.  
We assume $\gamma>\wtd\gamma_{\star}$, so that GS-SVM is feasible with probability approaching 1.

\noindent\textbf{Definitions:}~Following the notation introduced before Theorem \ref{thm:main_imbalance},
we let random variables as follows:
\begin{equation*}
\begin{cases}
~G\sim \Nn(0,1),\quad \text{$Y$ symmetric Bernoulli with $\Pro\{Y=+1\}=\pi$,}\\
~\text{$S$ takes values $1$ or $2$ with $\mathbb{P}\{S=1\}=p$,}
\end{cases}
\end{equation*}
\begin{equation*}
%\begin{cases}
~\wtd{E}_{S}=\eb_1\ind{S=1}+\eb_2\ind{S=2}\quad\text{and}\quad \wtd\Delta_S=\delta\cdot\ind{S=1} +1\cdot\ind{S=2},\quad\text{for}~\delta>0.
%\end{cases}
\end{equation*}
With these define the following functions $ \wtd\eta_\delta:\R_{\geq0}\times\Bc_2^{r}\times\R\rightarrow\R$ as \\
\begin{align*}
    \wtd\eta_\delta(q,\rhob,b)&:=\E\big[\big(G+\wtd E_{S}^T\Vb\Sb\rhob + \frac{bY-\wtd\Delta_S}{q}\big)_{-}^2\big] \nn- (1-\|\rhob\|_2^2)\gamma.
\end{align*}
Finally, define $(q_\delta,\rhob_\delta,b_\delta)$ as the \emph{unique} triplet satisfying $\wtd \eta_\delta(\wtd q_\delta,\wtd \rhob_\delta,\wtd b_\delta)= 0$ and 
$(\wtd \rhob_\delta,\wtd b_\delta):=\arg\min_{\substack{\|\rhob\|_2\leq 1, b\in\R}}\eta_\delta(q_\delta,\rho,b).$ Again, these triplets can be easily computed numerically for given values of $\gamma, \delta, \pi, p$ and means' Gramian $\M^T\M = \Vb\Sb^2\Vb^T.$


%In the SM, we show that $\eta_\delta,\wtd\eta_\delta$ are strictly convex with respect to $(\rhob,b)$ and that $$ Finally, 

%\begin{equation*}
%\begin{cases}
%%~G\sim \Nn(0,1), \quad \text{$Y$ symmetric Bernoulli with $\Pro\{Y=+1\}=\pi$}\\
%~\text{$S$ takes values $1$ or $2$ with $\mathbb{P}\{Y=1\}=p$}\\
%~E_{S}=\eb_1\ind{S=1}+\eb_2\ind{S=2}\quad\text{and}\quad\Delta_S=\delta\cdot\ind{S=1} +1\cdot\ind{S=2},
%\end{cases}
%\end{equation*} 
%and function $\wtd\eta_\delta:\R_{\geq0}\times\Bc_2^{r}\times\R\rightarrow\R$ as 
%$
%		%&\eta_\delta(\qt,\rhobt,\bt):=
%		\wtd\eta_\delta(q,\rhob,b):=\E\big(G+E_{S}^T\Vb\Sb\rhob + \frac{bY-\Delta_S}{q}\big)_{-}^2 \nn- (1-\|\rhob\|_2^2)\gamma.
%$



%\subsection{Analysis of CS-SVM}\label{sec:CS-SVM_sharp}


%\vp\noindent\textbf{Data model:}~For \emph{label-imbalances}, we consider a Gaussian mixture model (GMM) in which all examples belong to the same group (aka $K=1$). For the label $y\in\{\pm1\}$, we assume $\Pro\{y=+1\}=1-\Pro\{y=-1\}=\pi\in(0,1)$ and  $\pi<1-\pi$, so that class $+1$ is the minority class. The conditional of the feature $\x$ given its label $y$ is a multivariate Gaussian of mean $\mub_{y}\in\R^d$ and covariance $\Sigmab$, i.e.,
%$
%\x\big|y,\,\widesim{} \Nn(\mub_{y},\Sigmab).
%$
%We focus on the case $\Sigmab=\mathbf{I}_d$ and defer extensions to the SM.
%Let $\M=\begin{bmatrix} \mub_{+} & \mub_{-}\end{bmatrix}$ be the matrix of means and consider the eigen-decomposition of its Grammian:
%$
%\M^T\M = \Vb\Sb^2\Vb^T,~~ \Sb\succ \mathbf{0}_{r\times r},\Vb\in\R^{2\times r}, r\in\{1,2\},
%$
%with $\Sb$ an $r\times r$ diagonal positive-definite matrix and $\Vb$ an orthonormal matrix obeying  $\Vb^T\Vb=\mathbf{I}_r$. Finally, let $\eb_1=[1 \,,\, 0]^T$ and $\eb_2= [0 \,,\, 1]^T$ be the standard basis vectors in $\R^2$.

%%%\vspace{-0.05in}
%\noindent\textbf{Analysis of CS/GS-SVM:}~
%We first present a precise analysis of the balanced error of CS-SVM.  

%%\vspace{-0.1in}
%\begin{theorem}[Balanced error of CS-SVM]\label{thm:main_imbalance}
%%Consider data following the GMM with $K=1$, priors $(\pi, 1-\pi)$ and eigen-decomposition of Grammian matrix as in \eqref{eq:SVD}. 
%Let GMM data with label imbalances and learning regime as described above. 
%Consider the CS-SVM classifier in \eqref{eq:CS-SVM} with $h(\x)=\x$, intercept $b$ (i.e. constraints $\inp{\x}{\w}+b\geq\{\delta \text{ or } 1\}$ in \eqref{eq:CS-SVM}) and fixed margin-ratio $\delta>0.$ 
%%\so{What is $(\cdot)_-$ notation? Taking the negative part? So we take the squared of the negative part?}
%%Let $(q_\delta,\rhob_\delta,b_\delta)$ be the unique triplet satisfying
%%$\eta_\delta(q_\delta,\rhob_\delta,b_\delta)= 0$ and 
%%$(\rhob_\delta,b_\delta):=\arg\min_{\substack{\|\rhobt\|_2\leq 1, \bt\in\R}}\eta_\delta(q_\delta,\rhobt,\bt).$
%%and $\rhob_\delta,b_\delta$ be the corresponding unique minimizers of $\eta_\delta(q_\delta,\rhobt,\bt)$.  
%Define 
%$\Rco_+:=Q\left(\eb_1^T\Vb\Sb\rhob_\delta+b_\delta/q_\delta\right)$ and $\Rco_-:=Q\left(-\eb_2^T\Vb\Sb\rhob_\delta-b_\delta/q_\delta\right).$
%Then, in the limit of $n,d\rightarrow\infty$ with $d/n=\gamma>\gamma_\star$, it holds that 
%$\Rc_+\rP\Rco_+$ and $\Rc_-\rP\Rco_-$.
%In particular, 
%%the balanced error $\Rcbal$ converges in probability as follows:
%$\Rcbal\rP\Rcbalinf:=(\Rco_++\Rco_-)\big/2.$
%\end{theorem}
%%%\vspace{-0.1in}
%The theorem's proof further shows that the CS-SVM solution $\wh_\delta$ satisfies 
%$(\|\hat\w_\delta\|_2, \frac{\wh_\delta^T\mub_+}{\|\wh_\delta\|_2}, \frac{\wh_\delta^T\mub_-}{\|\wh_\delta\|_2} , \hat b_\delta) \rP (q_\delta,\eb_1^T\Vb\Sb\rhob_\delta,\eb_2^T\Vb\Sb\rhob_\delta, b_\delta).
%$
%Thus, $b_\delta$ is the asymptotic value of the intercept, $q_\delta^{-1}$ is the asymptotic value of the classifier's margin ${1}/{\|\wh_\delta\|_2}$ to the majority class, and $\rhob_\delta$ characterizes the asymptotic alignment of the classifier's hyperplane with the class means. The proof uses the convex Gaussian min-max theorem (CGMT) framework \cite{StojLAS,thrampoulidis2015regularized}; see SM for background, related works, the proof, as well as, (a) simpler expressions when the means are antipodal ($\pm \mub$) and (b) extensions to general covariance model ($\Sigmab\neq\mathbf{I}$). The experiment (solid lines) in Figure \ref{fig:mismatch_intro}(a) suggests the validity of the theorem's asymptotics predictions even at relatively small dimensions; see SM for additional experiments. %We also give experiments on MNIST dataset with theory-inspired $\delta$-tuning method.



%\begin{figure}[t]
%\begin{subfigure}[b]{0.55\textwidth}
%			\centering
%\includegraphics[width=0.8\textwidth,height=0.45\textwidth]{fig_bal_misclas_tradeoff_s=3_p_min=0p05.PNG}
%			\caption{}
%		\end{subfigure}
%\begin{subfigure}[b]{0.45\textwidth}
%			\centering
%\includegraphics[width=0.8\textwidth,height=0.52\textwidth]{fig_deo_vs_misclas_theory_fixed_s_priors_varying_gamma_alpha_s_min=3_s_maj=3_p_minor_class=0p5_p_minor_group=0p05.PNG}
%			\caption{}
%		\end{subfigure}
%	\caption{Trade-offs between misclassification error and error imbalance / balanced error / DEO on GMM data achieved by \textbf{(a)} CS-SVM for class prior  $\pi=0.05$ and \textbf{(b)} GS-SVM  for group prior $p=0.05$, as a function of the margin-ratio hyperparameter $\delta\geq 1$ and for different values of $\gamma$. The plots are generated using predictions of Theorems \ref{thm:main_imbalance} and \ref{thm:main_group_fairness}. See text for interpretations.
%	} 
%	\label{fig:tradeoffs}	
%\end{figure}


%%%\vspace{-0.05in}
%\noindent\textbf{Analysis of GS-SVM:}
%%%\vspace{-0.05in}
%Next, we characterize the DEO of GS-SVM. 
%Let $G,Y$ as defined in the previous paragraph. For $\delta>0$, define additional random variables as follows: 
%\begin{equation*}
%\begin{cases}
%%~G\sim \Nn(0,1), \quad \text{$Y$ symmetric Bernoulli with $\Pro\{Y=+1\}=\pi$}\\
%~\text{$S$ takes values $1$ or $2$ with $\mathbb{P}\{Y=1\}=p$}\\
%~E_{S}=\eb_1\ind{S=1}+\eb_2\ind{S=2}\quad\text{and}\quad\Delta_S=\delta\cdot\ind{S=1} +1\cdot\ind{S=2},
%\end{cases}
%\end{equation*} 
%and function $\wtd\eta_\delta:\R_{\geq0}\times\Bc_2^{r}\times\R\rightarrow\R$ as 
%$
%		%&\eta_\delta(\qt,\rhobt,\bt):=
%		\wtd\eta_\delta(q,\rhob,b):=\E\big(G+E_{S}^T\Vb\Sb\rhob + \frac{bY-\Delta_S}{q}\big)_{-}^2 \nn- (1-\|\rhob\|_2^2)\gamma.
%$
Although similar in nature, the result differs to Theorem \ref{thm:main_imbalance} since now each class itself is a Gaussian mixture. 

%%\vspace{-0.1in}
\begin{theorem}[DEO of GS-SVM]\label{thm:main_group_fairness}
Let group-sensitive GMM data  and learning regime as described above. 
Consider the GS-SVM classifier with $h(\x)=\x$, intercept $b$ and fixed margin-ratio $\delta>0$ (corresponding to group VS-loss with $\Delta_{y,g}=\Delta_{g}, g=1,2$ such that $\delta=\Delta_2/\Delta_1$).
%Consider the GMM with feature distribution and priors as specified in the `Data model' above. 
%	Let $(\wtd q_\delta,\wtd \rhob_\delta, \wtd b_\delta)$ be the unique triplet satisfying same equations as in Theorem \ref{thm:main_imbalance}, but with $\eta_\delta$ replaced with the function $\wtd \eta_\delta$ above. 
%	equation
%	\begin{align}\label{eq:eta_eq}
%		\min_{\substack{\|\rhobt\|_2\leq 1,\, \bt\in\R}}\eta_\delta(\qt,\rhobt,\bt) = 0\,,
%	\end{align}
%	and $\rhob,b$ be the unique minimizers of $\eta_\delta(q,\rhobt,\bt)$. 
Then, in the limit of $n,d\rightarrow\infty, d/n=\gamma>\wtd\gamma_{\star}$ it holds 
$
\Rc_{\pm,i} \rP Q\big({\eb_i^T\Vb\Sb\wtd \rhob_\delta\pm \wtd b_\delta/{\wtd q_\delta}}\big), i=1,2.$ In particular, 
%the difference of equal opportunity (DEO) satisfies 
$
\Rc_{\rm deo} \rP Q\big({\eb_1^T\Vb\Sb\wtd \rhob_\delta+ \wtd b_\delta/{\wtd q_\delta}}\big) - Q\big({\eb_2^T\Vb\Sb\wtd \rhob_\delta+ \wtd b_\delta/{\wtd q_\delta}}\big).$
\end{theorem}


==> underP.tex <==
\section{Underparameterized Regime}

%For simplicity assume here that $\mub_{+1}=-\mub_{-1}=-\mub$.

\ct{I did some guessing of the formulas here. Need to verify at some point.}

\begin{theorem}\label{thm:main_imbalance_underP}
Consider the Gaussian mixture data model in Section \ref{sec:data} with $K=1$, priors $(\pi, 1-\pi)$ for the two classes and eigen-decomposition of Grammian matrix of means as in \eqref{eq:SVD}. Let $(\wh,\bh)$ be the solution to the following ERM with logit-adjusted cost:
\begin{align}
\min_{\w,b}\frac{1}{n}\sum_{i\in[n]}\log\left(1+e^{\Delta_{y_i}} e^{-y_i(\x_i^T\w+b)}\right),
\end{align}
where $\Delta_{y_i}=\begin{cases}\Delta_{+1}&, y_i=1\\ \Delta_{-1}&, y_i=-1\end{cases}$. 
 Define random variables $G, Y, \Delta_Y\in\R$ and $E_Y\in\R^{2\times 1}$ as follows: $G\sim \Nn(0,1)$, $Y$ is a symmetric Bernoulli with $\Pro\{Y=+1\}=\pi$, $E_Y=\eb_1^T\ind{Y=1} - \eb_2^T\ind{Y=-1}$, and $\Delta_Y=\Delta_{+1}\cdot\ind{Y=+1} + \Delta_{-1}\ind{Y=-1}$. Finally, let $\Mc_{\ell}(\cdot;\la)$ be the Moreau envelope function at scale $\la$ of the sigmoid function $\ell(t)=\log(1+e^{-t}).$ Denote $\Mc_{\ell}^\prime(\cdot;\la)$ its derivative. With these, let $(q,\rhob,\la,b)\in\R_+\times\Sc^{r-1}\times\R_{+}\times\R$ be the unique solution to the following system of four equations in four unknowns:
 \begin{align*}
 \E\left[(G+q\,\eb_1^T\Vb\Sb\rhob)\cdot\Mc_{\ell,1}^\prime\left(qG+q\,\eb_1^T\Vb\Sb\rhob+bY-\Delta_Y;\la\right)\right] &= 0\\
  \la^2\E\left[\Mc_{\ell}^\prime\left(qG+q\,\eb_1^T\Vb\Sb\rhob+bY-\Delta_Y;\la\right)\right] &= \gamma q^2 (1-\|\rhob\|_2^2)\\
    \la\E\left[G\cdot\Mc_{\ell}^\prime\left(qG+q\,\eb_1^T\Vb\Sb\rhob+bY-\Delta_Y;\la\right)\right] &= \gamma q \sqrt{1-\|\rhob\|_2^2}\\
    \E\left[Y\cdot\Mc_{\ell}^\prime\left(qG+q\,\eb_1^T\Vb\Sb\rhob+bY-\Delta_Y;\la\right)\right] &= 0
 \end{align*}
 Then, in the limit of $n,d\rightarrow\infty$ with $d/n=\gamma<\gamma_\star$ it holds that
\begin{align*}
\Rc_{+} \rP Q\left(\eb_1^T\Vb\Sb\rhob+b/q\right)\text{ and }
\Rc_{-} \rP Q\left(\eb_2^T\Vb\Sb\rhob-b/q\right).
\end{align*}

\end{theorem}

